A Novel Side-Channel in Real-Time Schedulers

We demonstrate the presence of a novel scheduler side-channel in preemptive, fixed-priority real-time systems (RTS); examples of such systems can be found in automotive systems, avionic systems, power plants and industrial control systems among others. This side-channel can leak important timing information such as the future arrival times of real-time tasks.This information can then be used to launch devastating attacks, two of which are demonstrated here (on real hardware platforms). Note that it is not easy to capture this timing information due to runtime variations in the schedules, the presence of multiple other tasks in the system and the typical constraints (e.g., deadlines) in the design of RTS. Our ScheduLeak algorithms demonstrate how to effectively exploit this side-channel. A complete implementation is presented on real operating systems (in Real-time Linux and FreeRTOS). Timing information leaked by ScheduLeak can significantly aid other, more advanced, attacks in better accomplishing their goals.

==> Makefile <==
# Makefile for Latex
# Created by Sibin M.
# Date : May 15, 2004.

LATEX = pdflatex 
BIBTEX = bibtex
DVIPS = dvips
DVIPDF = dvipdf
PDFTOOO = pdf2oo -batch 
PSTOPDF = ps2pdf
PDFTOPS = pdf2ps
ACROBAT_COMPATIBILITY = 1.5

# MAIN_FILE_NAME = rtss09
MAIN_FILE_NAME = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex | gawk -F . 'BEGIN {filename;} /tex/ { filename = $$1; } END{printf(filename);}' )
BIB_FILES = mybib.bib realime.bib ada9x.bib sibin.bib power.bib zhu.bib arch.bib
# BIB_FILES := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

EMBED_SRC := $(MAIN_FILE_NAME)
EMBED_RESULT := $(MAIN_FILE_NAME)_embedded
EMBED = gs -sDEVICE=pdfwrite -q -dBATCH -dNOPAUSE -dSAFER -dPDFX -dPDFSETTINGS=/prepress -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode -dAutoFilterGrayImages=false -dGrayImageFilter=/FlateEncode -sOutputFile=$(EMBED_RESULT).ps -c '<> setdistillerparams' -f $(EMBED_SRC).ps -c quit

GOALS = $(MAIN_FILE_NAME).dvi

#%.pdf:  %.dvi
#	$(DVIPDF) $<
#	$(EMBED)

%.pdf:  %.ps
#	$(DVIPDF) $<
#	$(EMBED)
#	$(PDFTOPS) $(EMBED_RESULT).pdf 
#	cp $(EMBED_RESULT).ps $(EMBED_RESULT)_temp.ps
	$(EMBED)
	$(PSTOPDF) -dCompatibilityLevel=$(ACROBAT_COMPATIBILITY) -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter $(EMBED_RESULT).ps
	cp $(EMBED_RESULT).pdf $(MAIN_FILE_NAME)_submission.pdf


%.ps:	%.dvi
	$(DVIPS) -o $(MAIN_FILE_NAME).ps $<

%.odp:	%.pdf
	$(PDFTOOO) $(MAIN_FILE_NAME).pdf

%.dvi:	$(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

all: 	clean $(GOALS)

$(MAIN_FILE_NAME).dvi:	$(MAIN_FILE_NAME).tex
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

clean:
	rm -rf *.dvi *.log *.bbl *.blg *.aux *~

clobber:
	make clean
	rm -rf $(MAIN_FILE_NAME).pdf $(MAIN_FILE_NAME).ps $(MAIN_FILE_NAME).odt


==> Sections/analysis_probability.tex <==
\subsection{Probability Model}

In this section, we propose a probability model to evaluate the rate of correctly inferring the true arrival column (\ie the initial offset of the victim task).
Since the model requires more information about the system than what we assume the attacker knows, this model is not for the attacker.
Instead, we intend to give an approximate carry out massive experiments to give an approximate

As we introduced in Section~\ref{sec::infer_initial_offset}, the effectiveness of the algorithms relies on the number of blank intervals left in the end.
In other words, the more time columns we remove from the second step (Section~\ref{sec::analyze_ei}), the more likely we can get the correct inference.
Therefore, the process of the elimination of the time columns can be modeled as a probabilistic problem: what is the probability of a time column being removed from the inference?% as more execution intervals are constructed and placed on the schedule ladder diagram?
%Note that from Theorem we know that the true arrival column will always be blank and will not be removed, so here we only care about the probability of the removal for the time columns that are not true arrival column.

From Theorem~\ref{th:remove_flase_columns}, we know that the necessary condition to remove a time column is when an execution interval of the observer task appears.
This condition is satisfied if there exists an instant that corresponds to the time column when all tasks $\in hp(\tau_o)$ are inactive.
Therefore, the probability of all tasks $\in hp(\tau_o)$ are inactive at a time column is used to compute the probability of a time column being removed from the candidate list.

We first

% From Observation~\ref{observation:periodic_arrival}, we know that the arrivals of the victim task are fixed in the same time column (\ie the true arrival column $a_v$).


==> Sections/analysis_sporadic.tex <==

\subsection{Periodic Observer Task vs. Sporadic Observer Task}
The introduced algorithms can be applied to an observer task being either a periodic task or a sporadic task.
%The above theorems and algorithms can be applied to an observer task being either a periodic task or a sporadic task.
Yet, given the same target system, the latter may perform better than the former as the sporadic task naturally has more flexible arrivals which are constrained only by its minimum inter-arrival time.
A smart attacker who owns a sporadic observer task can exploit this advantage to adjust its inter-arrival time to increase the observation coverage against the victim task.
As a result, the introduced theorems depict the worst case condition for the sporadic task when it performs the attack with a constant inter-arrival time.
%Due to the space limit, we only focus on this most restricting condition.
%We plan to extend the \ATTCKNF algorithms in future work to take advantage of sporadic arrivals.  

\begin{comment}
\subsection{Observer Task: Real-time vs. Non-real-time}
\label{sec::observer_vs}
The \ATTCKNF algorithms can be applied to an observer task being either a real-time task or a non-real-time task since the computation only relies on the victim task's period.
Yet, given the same target system, the latter (non-real-time) performs better than the former as the real-time observer task is restricted by its real-time constraints.
This inference can also be drawn from the coverage ratio we discussed in Section~\ref{sec::determine_capability}.
The non-real-time observer task potentially has no limits on its coverage ratio as well as the maximum reconstruction duration $\lambda$ and is only limited by how long the attacker stays in the system.
In contrast, special care needs to be taken by the attacker when a periodic real-time observer task is engaged.
As a result, the introduced algorithms and theorems cover the worst case condition when carrying out the reconnaissance. %with a periodic real-time observer task.
\end{comment}

==> Sections/approach_analyzeEi__backup_.tex <==
%##### subsection #####
\subsection{Analysis of Execution Intervals}
\label{sec::analyze_ei}

Once the observer task's execution intervals are reconstructed, we 
analyze the data to extract the information about the victim task.
We do this by organizing the obtained execution intervals into a timeline split
into lengths of the victim task's period $p_v$
(recall that $p_v$ is one of the known quantities for the attacker).
%\footnote{Recall from Section~\ref{sec::adver_model} that this information is known to the attacker.}. 
The purpose of this step is to place
the execution intervals of the observer task within the periodic windows of the victim task.  
The timeline with length of the victim task's period allows the
attacker to see how the observer task's execution intervals are influenced by
the victim task as well as other higher-priority tasks.
%influences the observer task's execution (\ie the preemptions caused by the
%victim task).

To better illustrate the idea of the timeline and the proposed algorithms, we
will use a ``\emph{schedule ladder diagram}'' (defined below) to represent the
construction of the timeline in this paper. The rows in the schedule ladder diagram can
%, of course, 
be merged into a single-line timeline (and is just an analytical ``trick'').
%To organize the observed busy intervals and magnify the intervals induced by
%the victim task, we propose to use a \emph{schedule ladder diagram}.% that is
%defined as follows:
A schedule ladder diagram is a skeleton consisting of a set of
adjacent timelines of equal lengths -- that match the victim task's period
$p_v$. %(recall that the period of the victim task is one of the known quantities for the attacker). 
The start time of the top section can be an 
arbitrary point in time assigned by the attacker (\eg the time instant when the 
algorithms are first invoked).
%A set of given execution intervals, $W$, is plotted on such a configured
%skeleton. 
The columns in the schedule ladder diagram are ``unit time columns''. So, there are $p_v$ time columns. The skeleton of a schedule ladder diagram is illustrated in Figure~\ref{fig:ladder_example}.
%For simplicity, we will use the term \emph{schedule ladder diagram} to
%represent the \emph{schedule ladder diagram} plotted based on the victim
%task's period.
%
\begin{figure}[t]
%\vspace{-\baselineskip}
\centering
\includegraphics[width=0.65\columnwidth]{Figures/ladder_example}
\vspace{-0.5\baselineskip}
\caption{The skeleton of a schedule ladder diagram. It is used by the
	observer to organize its execution intervals. The start
	time $t$ of the schedule ladder diagram (\ie the beginning of the top
	timeline) is an arbitrary point in time, as assigned by the attacker. The width of each timeline
	matches the victim task's period $p_v$. The relative offset between the
	start time $t$ and the true arrival column is defined by $\ARRVCOL$.}
\label{fig:ladder_example}
\vspace{-1\baselineskip}
\end{figure}
%
\begin{comment}
% \begin{definition}
% (Schedule Ladder Diagram)
% A \emph{schedule ladder diagram}, formulated by $SLD(t_0, p)$, is a skeleton consisting of a set of adjacent time lines of which lengths are equal to the given period $p$.
% The start time of the top time line is assigned by the given $t_0$ which can be an arbitrary value.
% %A set of given execution intervals, $W$, is plotted on such a configured skeleton. 
% The columns in the \emph{schedule ladder diagram} are defined as ``time columns'' (so there are $p$ time columns). 
% \end{definition}

%The \emph{schedule ladder diagram} can be used to easier represent arrivals and execution intervals for a specific task.
%

% %because it is plotted based on the task's period.
% We use the following example to show how a \emph{schedule ladder diagram} can be used on the given task $\tau_v$.

% \begin{example}
% \label{example:ladder_diagram}
% Consider a simple system that has the task set $\Gamma=\{\tau_v, \tau_o\}$, $pri_v>pri_o$. The task parameters are given in the table below. 
% By inserting execution intervals of $\Gamma$ to the schedule ladder diagram $SLD(0, p_v)$, we can get the diagram shown on the right below.

% \begin{figure}[h]
% \vspace{-1\baselineskip}
% \centering
% \begin{minipage}{.4\columnwidth}
%   \centering
% \begin{tabular}{|c||c|c|c|}
% \hline 
%  & $p_i$ & $e_i$ & $a_i$ \\ 
% \hline %\hline 
% $\tau_v$ & 5 & 1 & 2 \\ \hline 
% $\tau_o$ & 7 & 1 & 0 \\ \hline 
% %\multicolumn{3}{r}{} \\
% \end{tabular} 
% \end{minipage}%
% %\hspace{.05\columnwidth}
% \begin{minipage}{.5\columnwidth}
%   \centering
% \includegraphics[width=0.75\columnwidth]{Figures/ladder_example}
% %\vspace{-0.5\baselineskip}
% \caption{An example of $SLD(0, p_v)$ with inserting execution intervals of $\Gamma=\{\tau_v, \tau_o\}.$}
% \label{fig:ladder_example}
% \end{minipage}
% %\vspace{-1\baselineskip}
% \end{figure}

% \end{example}
% In \emph{Example~\ref{example:ladder_diagram}}, we plot a schedule ladder diagram based on the $\tau_v$'s period $p_v$.
% From the arrivals of $\tau_v$, we have the following observation:
\end{comment}
%
From the diagram, plotted based on $p_v$, we make the
following observation:
\begin{observation}
\label{observation:periodic_arrival}
Any \emph{schedule ladder diagram} of a task $\tau_v$ must contain
exactly one arrival/execution instance of $\tau_v$ in every row.
%\footnote{Recall that each row represents an interval that matches one period of the victim task.}.
%Each arrival is located in each layer with the same offset.
All arrivals of $\tau_v$ are located in the same time column.
%The position of the arrival in each layer is the same.
%\qedsymbol
\end{observation}
% \begin{proof}
% Since $\tau_v$ is a periodic task, it arrives periodically every $p_v$ time.
% On the other hand, the execution ladder diagram of $\tau_v$ is plotted based on $p_v$, thus every layer (\ie every $p_v$) must contain one arrival from $\tau_v$.
% \end{proof}

This observation is true because $\tau_v$ is a periodic task that arrives every $p_v$ time units and the schedule ladder diagram is plotted with
its interval equal to $p_v$. We define the column where the arrivals of
the victim task are located as the ``true arrival column'', denoted by $\ARRVCOL$.  
%Since the column number of the true arrival column resembles the victim task's initial offset $a_v$ (from the start of the interval/row), we will use $a_v$ to represent the true arrival column for the simplicity of the expression. 
Thus, the correlation between the initial offset $a_v$ and the true arrival column $\ARRVCOL$ can be derived by $(t + \ARRVCOL - a_v) \ mod \ p_v = 0$, where $t$ represents the (arbitrary) start time of the schedule ladder diagram assigned by the attacker.
This is also depicted in Figure~\ref{fig:ladder_example}. 
%\todo[inline]{Rod: technically this is not correct. The correct relation is $(t + \ARRVCOL - a_v) \ mod \ p_v = 0$, because there is no guarantee that $a_v \leq p_v$. In your relation, either the left or right part could be $\geq p_v$. $\alpha$ and $a$ might also look too similar.}

The observation also means that the time columns $[\ARRVCOL, \ARRVCOL+bcet_v)$, where
$bcet_v$ is the best case execution time of $\tau_v$ (\ie the shortest possible execution time of $\tau_v$), will always be occupied
by either the victim task or other higher-priority task
executions. %(since they can preempt the victim task).
From this observation, 
we define the following theorem for placing the observer task's execution 
intervals on this schedule ladder diagram. 

\begin{theorem}
\label{th:blank_columns}
	The interval (time columns) $[\ARRVCOL, \ARRVCOL+bcet_v)$ does not contain any execution interval of the observer task. 
\end{theorem}
\begin{comment}
\begin{proof}
From Observation~\ref{observation:periodic_arrival}, the victim task $\tau_v$
	arrives regularly at time column $a_v$. Upon an arrival of $\tau_v$,
	it is scheduled to be executed at the arrival column/instant $\ARRVCOL$. If
	there exists lower priority tasks $lp(\tau_v)$ in execution at $\ARRVCOL$
	column, the victim task preempts such tasks until it finishes its job
	with length of $bect_v$ at a minimum. In the case that there exists
	higher priority tasks $hp(\tau_v)$ that are executing or arriving during
	$[\ARRVCOL, \ARRVCOL+bcet_v)$, the victim task $\tau_v$ is preempted. Under this
	circumstance, if the observer task $\tau_o$ had arrived during $[\ARRVCOL,
	\ARRVCOL+bcet_v)$, as a lower priority task, it is also preempted.
	Therefore, the time columns $[\ARRVCOL, \ARRVCOL+bcet_v)$ {\em cannot} contain the
	execution intervals of the observer task.
\end{proof}
\end{comment}

The proof of Theorem~\ref{th:blank_columns} is given in Appendix\ref{pf:blank_columns}. 
Note that $\ARRVCOL$ and $bcet_v$ are unknown to the attacker. If we place the
obtained execution intervals of the observer task on the schedule ladder
diagram and calculate the union of those execution intervals for every time column,
then, based on Theorem~\ref{th:blank_columns}, there must exist an empty
interval of continuous time columns of which the length is equal to or greater
than $bcet_v$. Here, an empty interval represents the time columns where the
observer task is always inactive and hence do not contain any execution intervals
of the observer task. Those empty time columns are candidates for containing
the true arrival time of the victim task. There may also exist time columns
that are empty %due to the preemptions 
due to other higher-priority tasks.
Yet, since other tasks have distinct arrival periods (or random arrivals for
real-time sporadic tasks and non-real-time tasks), those empty time columns tend to be scattered, compared to $[\ARRVCOL, \ARRVCOL+bcet_v)$, and are expected
to be eliminated as more execution intervals of the observer task are collected. 
In practice, our results indicate that this process works effectively and is mostly stabilized after an attack duration of $5 \cdot LCM(p_o,p_v)$.
%
To this end, it's easier to think of the problem as the process of eliminating 
those time columns that are not true arrival columns for the victim. We use the following theorem 
to remove these ``false'' time columns.%intervals (\ie time columns -- we use intervals and time columns interchangeably for simplicity. Where necessary, we will differentiate between the two).
\begin{theorem}
\label{th:remove_flase_columns}
The time columns in which there exists at least one execution interval of 
	the observer task {\em cannot} be true arrival columns. %\qedsymbol
\end{theorem}
\begin{comment}
\begin{proof}
From Theorem~\ref{th:blank_columns}, the observer task is always preempted
	within time columns $[\ARRVCOL, \ARRVCOL+bcet_v)$. In other words, the execution
	intervals of the observer task can only appear at time columns $[0,
	\ARRVCOL)$ and $[\ARRVCOL+bcet_v,p_v)$. Therefore, the execution intervals of
	the observer task will not be present at the true arrival column ($\ARRVCOL$) and also it would have been preempted.
\end{proof}
\end{comment}
The proof of Theorem~\ref{th:remove_flase_columns} is presented in Appendix\ref{pf:remove_flase_columns}.
%A probability analysis is given in Section~REF.
Based on Theorem~\ref{th:remove_flase_columns}, we can remove corresponding
time columns when an execution interval of the observer is placed on the schedule ladder
diagram. Ultimately, the attacker can eliminate most of the false time columns,
thus leaving only a small portion of the time columns (containing $[\ARRVCOL, \ARRVCOL+bcet_v)$ based on Theorem~\ref{th:blank_columns}) to infer the victim task's
initial offset. %(\ie by inferring the true arrival column). 
The algorithm to
infer the victim task's initial offset 
%from the obtained empty time columns 
is introduced next. 
%It is worth mentioning that a known issue that weakens this method is when there exists tasks that are {\em harmonic} with the victim task\footnote{Harmonic tasks are those ones whose periods are multiples of one another -- hence, their executions can potentially overlap during certain intervals (rows in the scheduler ladder diagrams) thus making it harder to differentiate between the victim tasks and ones it shares harmonic periods with.}. In such cases, there could be more than one blank interval caused by the harmonic tasks that can not be eliminated. We can still analyze systems with harmonic task sets, but the precision of the final inference will drop.
%
%\todo{Move Example 1 to Appendix.}
%\hl{To help understand the aforementioned steps,} an example is given in Appendix\ref{sec:examples}.

\begin{comment}%Moved to Appendix (for RTAS'19)
\begin{example}
\label{example:analyze_ei}
Consider a system that has the real-time task set $\Gamma=\{\tau_1, \tau_o,
	\tau_v, \tau_4\}$. For the sake of simplicity, we assume that all 
	tasks are periodic tasks in this example (though our analysis can
	work with periodic, sporadic and mixed systems as well). The task 
	parameters are presented in the table below (on the left).
	Note that $pri_i > pri_j$ means that $\tau_i$ has a higher number 
	that $\tau_j$. Thus, task $\tau_1$ has the lowest priority while 
	task $\tau_4$ has the highest priority and $\tau_v$ has higher priority 
	than $\tau_o$. Let the maximum reconstruction duration $\BUDGET$ be $1$ 
	and the start time of the attack be $0$ (as a result, $a_v$ equals $\ARRVCOL$ in this example).  Assuming the attacker has 
	executed the first step/algorithm for some duration, the table 
	below lists the reconstructed execution intervals 
	of the observer task.
% By inserting execution intervals of $\Gamma$ to the schedule ladder diagram $SLD(0, p_v)$, we can get the diagram shown on the right below.

\begin{center}\footnotesize
\vspace{-0.8\baselineskip}
\begin{tabular}{|c||c|c|c|c|}
\hline 
 & $p_i$ & $e_i$ & $a_i$ & $pri_i$\\ 
\hline \hline 
$\tau_1$ & 15 & 1 & 3 & 1 \\ \hline 
$\tau_o$ & 10 & 2 & 0 & 2 \\ \hline 
$\tau_v$ & 8 & 2 & 1 & 3\\ \hline
$\tau_4$ & 6 & 1 & 4 & 4 \\ \hline 
%\multicolumn{3}{r}{} \\
\end{tabular} 
%\end{center}
%\vspace{-0.10in}
\quad
%\begin{center}\footnotesize
\begin{tabular}{|c|}
\hline 
Reconstructed \\ 
Execution Intervals \\ 
\hline \hline 
[0,1) \\ 
\hline 
[12,13) \\ 
\hline 
[20,21) \\ 
\hline 
[30,31) \\ 
\hline 
[43,44) \\ 
\hline 
\end{tabular} 
\vspace{-0.5\baselineskip}
\end{center}

Note that since $\tau_1$ has priority lower than the observer task $\tau_o$, it
does not influence the execution of $\tau_o$. Then, we place
the reconstructed execution intervals in a schedule ladder diagram of
width equal to the victim task's period $p_v$. This operation is shown in Figure~\ref{fig:ei_and_union_example}(a). 
To better understand the effectiveness of the schedule ladder diagram in profiling the victim task's behavior, we plot the original, complete, schedule  on the ladder diagram in Figure~\ref{fig:schedule_on_ladder_example} in Appendix so that readers get a better sense of it. 
This gives us an insight into the relation between the execution intervals of $\tau_o$ and that of the victim task.

\begin{figure}[t]
	\vspace{-1\baselineskip}
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.6\columnwidth]{Figures/ei_on_ladder_example}
        \vspace{-0.5\baselineskip}
        \caption{Placing the reconstructed execution intervals in the schedule ladder diagram.}
        \label{fig:ei_on_ladder_example}
	%\label{fig:arrv_seg_a}
        \vspace{-0.8\baselineskip}
    \end{subfigure}%   
    \hfill  
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.6\columnwidth]{Figures/union_example}
        \vspace{-0.5\baselineskip}
        \caption{Calculating union of the reconstructed execution intervals.}
        \label{fig:union_example}
        %\vspace{-0.5\baselineskip}
	%\label{fig:arrv_seg_b}
    \end{subfigure}
    \vspace{-0.8\baselineskip}
    \caption{Creating the schedule ladder diagram for Example~\ref{example:analyze_ei}.}
    \label{fig:ei_and_union_example}
    \vspace{-1.7\baselineskip}
\end{figure}

From the schedule ladder diagram in Figure~\ref{fig:ei_and_union_example}(a), 
we perform a {\em union of the execution intervals in each time column}. 
The results are shown in Figure \ref{fig:ei_and_union_example}(b) -- essentially 
a set of execution intervals and empties.
%The result is displayed in Figure~\ref{fig:union_example}.
%What left in this step is a set of execution intervals and blank intervals as
%shown in Figure~\ref{fig:union_example}.  
The empty intervals (\ie ones without execution intervals) are candidate
time columns that contain the true arrival column we want to extract. These 
empty intervals are passed to the final step to infer the initial offset/arrival times
of the victim task.\qedsymbol

\end{example}
\end{comment}



% ---------------------------------------

\begin{comment}


%Now let's consider $\tau_v$ to be the victim task and $\tau_o$ to be the observer task in the \emph{Example~\ref{example:ladder_diagram}}.
Now let's consider the \emph{observability} between the observer task $\tau_o$
	and the victim task $\tau_v$ in a \emph{schedule ladder diagram}, we
	can derive the following corollary from
	\emph{Theorem~\ref{th:observable}}:

%Now we insert the observed busy intervals $W_o$ into the execution ladder diagram.
%The effect of this operation relies on the following corollary:

\begin{corollary}
\label{corollary:overlap}
If the condition in Theorem~\ref{th:observable} is true (\ie $\tau_v$ is
	observable by $\tau_o$) in a infinite observation, then by inserting
	the observed busy intervals to the \emph{schedule ladder diagram},
	there must exist observed busy intervals that overlap the time column
	where the victim task's arrivals take place.
\end{corollary}
\begin{proof}
It is a result of Theorem~\ref{th:observable} presented in the \emph{schedule
	ladder diagram}.  Furthermore, since the observation is infinite, the
	condition in Theorem~\ref{th:observable} happens repeatedly (but not
	necessarily periodically).
\end{proof}


\begin{example}
\label{example:overlap}
Consider a simple system that has the task set $\Gamma=\{\tau_o, \tau_v,
	\tau_h\}$. The task parameters are given in the top left table below.
	Their task priorities are assigned by using the rate-monotonic
	algorithm.  The bottom left table on the left lists the first few busy
	intervals observed by $\tau_o$ using Algorithm~\ref{algo:observe_bi}.
	The figure on the right displays the schedule ladder diagram with
	inserting the observed busy intervals.  This shows that the busy
	interval $\omega_{o, 0}=[7,9)$ overlaps the victim task's arrival (\ie
	the second time column). 

\begin{figure}[h]\footnotesize
\vspace{-1\baselineskip}
\centering
\begin{minipage}{.4\columnwidth}
\centering
\begin{tabular}{|c||c|c|c|}
\hline 
 & $p_i$ & $e_i$ & $a_i$ \\ 
\hline %\hline 
$\tau_o$ & 7 & 1 & 0 \\ \hline 
$\tau_v$ & 6 & 1 & 1 \\ \hline 
$\tau_h$ & 5 & 1 & 3 \\ \hline 
\multicolumn{4}{r}{} \\ % This is just an empty line
\end{tabular} 

  \centering
\begin{tabular}{|r l|}
\hline 
\multicolumn{2}{|c|}{Observed $W$ by $\tau_o$} \\ \hline %\hline 
$\omega_{o,0}$ & $=[7, 9)$ \\ \hline 
$\omega_{o,1}$ & $=[14, 15)$ \\ \hline 
$\omega_{o,2}$ & $=[28, 29)$ \\ \hline 
\multicolumn{2}{c}{$\vdots$} \\ 
%\multicolumn{3}{r}{} \\
\end{tabular} 
\end{minipage}%
%\hspace{.05\columnwidth}
\begin{minipage}{.5\columnwidth}
  \centering
\includegraphics[width=0.9\columnwidth]{Figures/ladder_example_bi}
%\vspace{-0.5\baselineskip}
%\caption{TBD}
\label{fig:overlap_example}
\end{minipage}
%\vspace{-1\baselineskip}
\end{figure}

\end{example}


\end{comment}


==> Sections/eval_platform.tex <==
% \clearpage
% \newpage
%\section{Evaluation with Attack Demonstration}
\section{Motivating Use Cases}
\label{sec::eval_platform}
The \ATTCKNF algorithms are implemented on two operating systems with a real-time scheduling capability: \ci Real-Time Linux (\ie Linux with the PREEMPT\_RT patch)~\cite{RTLinux} and \cii FreeRTOS~\cite{FreeRTOS}.
%While the simulation-based experiments focus on the scalability of the algorithms, 
We first aim to demonstrate the feasibility of such algorithms on realistic platforms in this section.
%
\begin{comment}
Before delving into the demonstrations, we would like to point out that, as mentioned in the adversary model in Section~\ref{sec::adver_model}, 
we assume that the attacker has control of at least one task in the victim system in the demonstrations below.
%In both attack scenarios, we assume 
It can be accomplished by either compromising an existing task or by legitimately owning
a task in a system based on the multi-vendor development model~\cite{embeddedsecurity:mohan2015} which is a common practice for complex control systems.
Further, some work have demonstrated that real-time systems like commercial drones may contain critical design flaws and hence the root access may be compromised~\cite{pleban2014hacking,samland2012ar}.
In particular, RTS with a Linux kernel is arguably prone to attack due to its complexity.
Many vulnerabilities in Linux systems are discovered by researchers once a while.
Specifically, $12.8\%$ of the vulnerabilities can potentially help the attackers gain privileges and create an observer task. For instance, CVE-2017-10661, CVE-2017-7374, CVE-2017-7541, \etc, just to name a few from recent CVE disclosure~\cite{CVE}.
While there exist many other measures to get access to the observer task, the details are beyond the scope of this paper.
\end{comment}
%
In what follows, two attack cases are presented.
%All of them 
They benefit from the information obtained by the proposed algorithms since they learn critical time points in the schedule and better utilize such information to accomplish their primary attack goals.
The demo videos for the attacks can be found at \url{https://scheduleak.github.io/}.


\Note The main/novel contribution of this paper is the discovery of the scheduler side-channels in real-time autonomous control systems and the development of the \ATTCKNF algorithms described thus far. The attacks in Sections \ref{sec:take_over_the_control} and \ref{sec:cache_timing_attack} are just {\em examples} that show {\em how to use the extracted side-channel information} to improve the fidelity/success of other attacks and is not intended to demonstrate complete end-to-end attacks against such systems.

%\subsection{Taking Over Control of Autonomous Vehicles}
\subsection{Reducing Attack Overheads}
%\subsection{Interleaving Control Signals}
\label{sec:take_over_the_control}


Let's consider a real-time autonomous subsystem that controls some actuators.
The attacker wants to be able to override the control -- for the purpose of creating an illusion of bad control by causing (temporary or permanent) misbehavior or even taking over the control of the system for a short time span.
A brute force strategy of excessively overriding the control signals will not work in this scenario because its high attack overhead can cause some real-time tasks to miss their deadlines and lead to system failures.
Therefore, utilizing information from reconnaissance attacks like \ATTCKNF to help reduce attack overhead is particularly crucial when attacking a system containing real-time tasks.
%Arguably there are many ways to compromise the system and disable its functionality.
%However, for those attackers who want to stay undetected and sometimes create an illusion of bad control by causing a temporary misbehavior or even stealthily interleave the control of the actuators for a short time span, it isn't that straightforward.

Specifically, let's consider a remotely controlled rover or a quadcopter.
This type of systems is typically equipped with one or more electronic speed controllers (ESCs) and servos that receive pulse-width modulation (PWM) signals from the control board to drive its motors or actuators (\eg wheels, propellers, steering).
%To keep the PWM updated with the latest desired output value, a periodic real-time task is usually employed to submit the PWM value to hardware.
A periodic real-time task is usually used to update the PWM value in the hardware.
For example, the rover system we use in this demonstration has a periodic real-time task running at $50Hz$ (period is $20ms$).
Its job is to periodically update the PWM output as displayed in Figure~\ref{fig:exp_pwm_override}(a).
Since this actuator refresh rate (\ie $50Hz$ or $400Hz$) is commonly used in a control system, the attacker can easily infer the period of such tasks from publicly available information.

Figure~\ref{fig:exp_pwm_override}(b) and (c) show that the PWM output may be overridden by overwriting it with a different value to the PWM hardware block.
However, without exact schedule information, the attacker can either send the updates at random instants (Figure~\ref{fig:exp_pwm_override}(b)) or periodically but at an arbitrary offset that leads to ineffective attacks. 
%a careless attacker who randomly issues the PWM update may not lead to the same effect.
On the other hand, Figure~\ref{fig:exp_pwm_override}(c) displays that the attacker can carefully issue an PWM update {\em right after the original update} to override the PWM output. 
By doing so, an attacker can potentially take over control of the actuators. % behind the ESCs.
Yet, precise {\em future timing} knowledge of such a task is required to accomplish this goal. 
%It's also worth mentioning that the brute-force approach that excessively override the PWM output does not work in this scenario as it will consume a high CPU and peripheral utilization and increase chance of being detected.

% The second attack scenario aims to take over control of the system's actuators.
% Specifically, let's consider a remote controllable drone.

% A crucial point in this scenario is that the attacker wants to stealthily disturb the service (\ie the control of the actuators) and cause a temporary lost of controllability.
% cause illusion 
% This is useful when 
% 




\subsubsection{Setup}
%Linux navio 4.9.45-94f47ec-emlid-v7+ #4 SMP PREEMPT Wed Aug 30 18:17:43 MSK 2017 armv7l
We implement this attack on a real remote rover and a quadcopter.
%We use a real, custom remote rover to demonstrate the aforementioned attack. 
To illustrate, we will focus on the case of the rover here.
Its control system is built with a Raspberry Pi 3 Model B board~\cite{RaspberryPi}. 
A Navio2 module board~\cite{Navio2} that encapsulates various inertial sensors is attached to the Raspberry Pi board to enable the control capability.
The board is configured to use only a single core to match the assumed system model.
The system runs Real-Time Linux (\ie Raspbian, kernel 4.9.45 with PREEMPT\_RT patch) with an APM flight stack~\cite{Ardupilot} that is one of the most popular open-source code stack in the remote control community.
It consists of a set of real-time tasks to perform control-related jobs such as refreshing GPS coordinates, decoding remote control commands, performing PID calculation and updating output signals.
As mentioned earlier, we are targeting the task that periodically updates the PWM output (\ie the victim task with $p_v=20ms$).
The victim task handles two PWM output channels for steering and throttle.
%four motors (since it is a quadcopter).
In this attack, we intend to override both PWM output channels.

We assume that the attacker has got into the system, as we explained in Section~\ref{sec::adver_model}.
%Again, we assume that the attacker has got into the system with exploiting some existing vulnerabilities.
%Differing from the previous case, 
Here, we restrict the observer's capability to a non-real-time process in Linux.
%It is to explore the feasibility of using a sporadic task against a real-time victim task.
As a result, the observer task has the priority lower than all the real-time tasks in the system.
%Both the reconnaissance attack and overriding the PWM output are done in the observer task.
In this implementation, the observer task uses a system call, $\mathtt{clock\_gettime()}$, to obtain clock counts from $\mathtt{CLOCK\_MONOTONIC}$ to measure and reconstruct its own execution intervals. %the length of preemptions. 
%For ease of demonstration, the primary attack that overrides the PWM output is implemented as a separate program. They can be merged as one process without problems.

\begin{figure}[t]
	%\vspace{-1\baselineskip}
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.8\columnwidth]{Figures/exp_pwm_override_a}
        \vspace{-0.5\baselineskip}
        \caption{PWM output without the presence of an attack.}
	%\label{fig:arrv_seg_a}
        \vspace{0.3\baselineskip}
    \end{subfigure}%   
    \hfill  
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.8\columnwidth]{Figures/exp_pwm_override_b}
        \vspace{-0.5\baselineskip}
        \caption{PWM output overridden at random instants.}
	%\label{fig:arrv_seg_b}
    \vspace{0.3\baselineskip}
    \end{subfigure}
    \hfill  
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.8\columnwidth]{Figures/exp_pwm_override_c}
        \vspace{-0.3\baselineskip}
        \caption{PWM output overridden at precise time instants.}
        %\vspace{-0.5\baselineskip}
	%\label{fig:arrv_seg_b}
    \end{subfigure}
    \vspace{-1\baselineskip}
    \caption{An illustration of a PWM channel output on a rover system. The PWM output is updated periodically by a $50Hz$ task. (b) shows that an naive attack issuing the PWM updates at random instants may not be effective. (c) shows that the PWM output can be overridden by carefully issuing the PWM update right after the original update. }
    \label{fig:exp_pwm_override}
    \vspace{-1\baselineskip}
\end{figure}


\subsubsection{Attack Manifestation and Results}
The attack begins after the rover starts moving.
We let the observer task run the \ATTCKNF algorithms for 1 second and it successfully infers the victim task's arrival time with a precision of $99.85\%$ (defined formally in Section~\ref{sec::eval_metrics}).
Utilizing this precise schedule information, the attacker submits the forged PWM output only after the inferred time instants as shown in Figure~\ref{fig:exp_pwm_override}(c).
%As a result, the attack works as expected, results show that 
By probing the PWM signals, we observe that the overridden PWM signals are active $85\%$ of the time.
As a result, we see that the rover no longer responds to the remote controller. Instead, the rover is driven by the attacker's commands.
%Furthermore, the remote unsurprisingly shows no control of the quadcopter during the attack.
To further reduce the attacker's footprint, the attacker's task remains idle between two PWM updates, which leads to a CPU utilization of $2.6\%$.
As a comparison, a brute-force approach takes up $77.9\%$ CPU utilization (\ie all available CPU resource) to achieve the same effect.
%
% Comment out DOS demo to avoid confusion to the readers.
%\todo{Comment out DOS demo to avoid confusion to readers}
\begin{comment}
\subsection{Denial of Service Attack}
The same attack is also carried out on a real, custom quadcopter with the same control platform (\ie Raspberry Pi and Navio2). The quadcopter has relatively complex design with four ESCs controlled by four PWM output channels refreshing at a rate of $400Hz$. 
The concept of the attack is the same as shown in Figure~\ref{fig:exp_pwm_override}.
Differing from the previous attack where we try to take over the control, here we intend to demonstrate the denial of service attack with a low footprint.

The attack begins after the quadcopter takes off.
Similarly, we let the observer task run the reconnaissance algorithms for 1 second.
It produces an inference precision of $99.97\%$ (defined in Section~\ref{sec::eval_metrics})..
Then, we utilize the inferred time information to override the PWM outputs of the four motors.
As a result, the quadcopter becomes unbalanced and does not respond to the control commands from the remote controller nor from the ground control station. 
The attack leads to a CPU utilization of $17.8\%$ (the value is higher than the rover one because it requires a larger refresh rate, \ie $400Hz$).
Since the footprint is low, the system administrator may not be able to figure out the root cause immediately before the attacker leaves the system.
As a comparison, a brute-force approach takes up to $69.1\%$ CPU utilization to achieve the same effect.
\end{comment}
%
\begin{comment}
We let the observer task run the reconnaissance attack for 1 second and it successfully infers the victim task's arrival time with a inference precision of $99.97\%$.
Utilizing such precise schedule information, the attacker submits the forged PWM output only after the inferred time instants as introduced in Figure~\ref{fig:exp_pwm_override}(c).
%As a result, the attack works as expected, results show that 
By probing the PWM signals, we observe that the overridden PWM signals are active $72\%$ of the time.
As a result, we can see that the quadcopter becomes unbalanced and does not react to the remote controller nor the commands from the ground control station during the attack. 
%Furthermore, the remote unsurprisingly shows no control of the quadcopter during the attack.
To further reduce the attack's footprint, the attacker's task remains idle between two PWM updates, which leads to a CPU utilization of $17.8\%$.
As a comparison, a brute-force approach takes up $69.1\%$ CPU utilization (\ie all available CPU resource) to achieve the same effect.
\end{comment}







\subsection{Increasing Attack Precision}% of Cache-Timing Side-Channel Attacks}
\label{sec:cache_timing_attack}
%What follows presents the details of the motive attack described in Section~\ref{sec::intro}.
Here, we present the attack introduced in Section~\ref{sec::intro}.
A UAV executing a surveillance mission is considered. It captures high resolution images when flying over locations of interest.
%Let's consider an unmanned aerial vehicle (UAV) executing a reconnaissance mission is considered.
%The UAV's target is to fly over some territory and take high resolution photos when it reaches locations of high-interest.
%In this case, the attacker's goal is to not crash the UAV.
In this case, the attacker's goal is to stealthily learn the locations targeted by the UAV.
%Rather, the attacker wants to stealthily learn the locations of high-interest targets (where the surveillance camera on the UAV is enabled).
%Here, we mainly focus on the attacker's objective of learning locations of high-interest targets where the surveillance camera on the UAV is enabled.
%This can be done by monitoring the memory usage of the task that handles the pictures taken by the on-system surveillance camera.
The strategy is to monitor when the surveillance camera on the UAV is switched to a execution mode in which high-resolution images are being processed.
This can be done by exploiting a cache-timing side-channel attack to gauge the coarse-grained memory usage behavior of the task that handles the images (victim).
A high cache usage by the victim task would indicate that a high-resolution image is being processed, otherwise it would use less cache memory.
%In particular, we intend to exploit the cache-timing side-channel attack against such a task.
However, a random sampling of the cache will result in noisy (and often useless) data since there exist other tasks in the system. 
%it is infeasible without knowing when the task is scheduled to run because a random sampling of the cache will result in noisy -- often useless, data, as we show.
In contrast, knowing when the task is scheduled to run allows the attacker to execute prime and probe attacks \cite{osvik2006cache, page2002theoretical} very close to the victim task's execution.
As a result, a scheduler side-channel attack like the one presented in this paper that learns the schedule timing information is needed. 
%To extract clean memory usage quietly, a series of cache timing attacks launched at precise time instants is required.
In what follows, both, the results with and without information from \ATTCKNF, 
%the knowledge of the precise time information 
are demonstrated.





\subsubsection{Setup}
We use a Zedboard running the FreeRTOS OS to simulate the control system on a UAV.
The demonstration is done using hardware-in-the-loop (HIL) simulation where the system is attached to a computer for the flight route and to display its trajectory.
%
The system consists of an image processing task handling photos at a rate of $30Hz$ (\ie the victim task, $p_v=33ms$, which is known to the attacker) and four other real-time tasks (unknown to the attacker) -- all running in a periodic fashion.
%
The victim task reacts differently based on a preloaded list of GPS coordinates that are of interest to the victim.
It processes a large size of data when the UAV reaches a coordinate on the list.
%
Other real-time tasks consume differing amounts of memory.
%
We assume that the attacker enters the system as one of the low-priority periodic tasks (\ie the observer task, $p_o=40ms$) by exploiting some existing vulnerabilities.
%We assume that the attacker has got into the system as one of the low priority tasks (\ie the observer task, $p_o=40ms$), as we explained in Section~\ref{sec::adver_model}.
%While there exist many work studying how an UAV can be compromised (\eg XXXX), this is out of this paper's scope.
Here, the observer task is used to run both the \ATTCKNF attack and the cache-timing side-channel attack.
The observer task uses a 64-bit Global Timer (GT) that is shared in FreeRTOS on Zedboard to measure and reconstruct its own execution intervals. %the preempted intervals. 
%
We further assume that the attacker is able to obtain GPS coordinates via other means.
%It is not uncommon because, as we see from the previous attack case, most peripherals are typically not secure.
%
Ultimately, the attacker's goal is to combine the inference of the victim task's behavior and the obtained GPS coordinates to identify the locations of high-interest along the flight path.




\subsubsection{Attack Results}
First, let's consider an attacker who does not have access to \ATTCKNF-ed information.
The attacker launches the cache-timing side-channel attack at arbitrary instants due to a lack of precise timing information.
As shown in Figure~\ref{fig:cache_attack_probes}(a), this produces many cache probes (it is hard to distinguish the cache usage of the victim task from other tasks in Figure~\ref{fig:cache_attack_probes}(a)) and results in an unsuccessful attack. 
%shows the results of the cache timing attack under such a condition. demonstrates that a careless attacker who launches the cache timing attack at arbitrary instants may lead to many indistinguishable cache probes and result in an unsuccessful attack. 

\begin{figure}[t]
	%\vspace{-1\baselineskip}
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.69\columnwidth]{ExpFigures/CacheAttack_without_ScheduLeak}
        \vspace{-0.5\baselineskip}
        \caption{Attack without \ATTCKNF's assist.}
	%\label{fig:arrv_seg_a}
        %\vspace{-\baselineskip}
    \end{subfigure}%   
    \hfill  
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.69\columnwidth]{ExpFigures/CacheAttack_with_ScheduLeak}
        \vspace{-0.5\baselineskip}
        \caption{Attack with \ATTCKNF's assist.}
        %\vspace{-0.5\baselineskip}
	%\label{fig:arrv_seg_b}
    \end{subfigure}
    \vspace{-1\baselineskip}
    \caption{Results of the cache-timing side-channel attacks %introduced 
    in Section~\ref{sec:cache_timing_attack}. 
    %X-axis is the elapsed time in seconds and Y-axis is the cache-miss count measured by the attackers. 
    (a) demonstrates that a random mechanism launching the attack at arbitrary instants will lead to many indistinguishable cache usage results. (b) shows a successful attack in which four camera activation events (numbered by $1$ to $4$) are identified from the cache probes using precise time information inferred by \ATTCKNF. }
    \label{fig:cache_attack_probes}
    %\vspace{-0.2\baselineskip}
\end{figure}

%\todo{Move the map to Appendix.}
%\begin{comment}
\begin{figure}[t]
%\vspace{-\baselineskip}
\centering
\includegraphics[width=0.59\columnwidth]{ExpFigures/cache_timing_attack_gps_trace_w_legend}
\vspace{-0.8\baselineskip}
	\caption{
    Data 
    %plotted on Google Map 
    recorded by the HIL simulator for the attack  in Figure~\ref{fig:cache_attack_probes}(b). 
    The bold line is the UAV's trajectory, the green circles represent the true locations-of-interest to the UAV, and the red pins (numbered by $1$ to $4$) are the high-interest locations inferred by the attacker. The result shows that the attacker's inference matches the ground truth. 
%The black numbering is mapped to that in Figure~\ref{fig:cache_attack_probes}(b).
}
\label{fig:cache_attack_gps_trace}
\vspace{-0.8\baselineskip}
\end{figure}
%\end{comment}

Then, we launch an attack after running \ATTCKNF attack in advance.
The \ATTCKNF attack algorithms run at the beginning to learn the victim task's future invocations.
In this case, the algorithms yield a precision of $99.998\%$  for the inference of the victim task (see Section~\ref{sec::eval_metrics} for the definition).
Once the analysis is complete, the attacker moves to the next stage to monitor the victim task's memory usage behavior.
With the precise schedule information, the attacker is able to launch the cache-timing side-channel attack right before and after the victim is executed and skip those instants that are irrelevant.
Figure~\ref{fig:cache_attack_probes}(b) shows the result of the precise cache probe against the victim task.
We see that the attack greatly reduces the noise caused by other real-time tasks and is able to precisely identify the victim task's memory usage behavior.
%
The attacker can therefore determine that the camera is activated if the victim task's memory usage is high or deactivated if the memory usage is low.
As a result, four camera activation instants can be identified from the spikes shown in Figure~\ref{fig:cache_attack_probes}(b).
Combining this with the real-time GPS data, the locations of high-interest can be uncovered.
Figure~\ref{fig:cache_attack_gps_trace} %(Appendix~\ref{sec::cache_attack_gps_trace})%given in \hl{Appendix}~\ref{sec::cache_attack_gps_trace} 
shows the UAV's trajectory, actual locations of interest (red markers) and the attacker's estimated points of interest (green dots).
The results suggest that the attack is successful and the \ATTCKNF attack can increase the effectiveness of the %primary attack (\ie the cache-timing side-channel attack) in achieving its goal.
cache-timing side-channel attack in achieving its goal.
%


==> Sections/intro_NDSS19.tex <==
%##### subsection #####
\section{Introduction}
\label{sec::intro}

\begin{figure*}[t]
%\vspace{-\baselineskip}
\centering
\includegraphics[width=0.95\textwidth]{Figures/paper_overview}
%\vspace{-0.7\baselineskip}
\caption{Overview of paper: We demonstrate how an unprivileged, low-priority task (in user space) can use the \ATTCKNF algorithms to infer execution behaviors of critical, high-priority real-time task(s). %the precise details of the victim task's schedule with an unprivileged task.
The extracted information is useful for helping other attacks achieve their primary goals (two such attack instances are implemented in this paper as possible use cases).
%Two instances of attack enabled by \ATTCKNF are implemented in this paper to demonstrate possible use cases of the extracted side-channel information. %damage from using the information provided by the \ATTCKNF algorithms.
}
\label{fig:paper_overview}
\vspace{-1.7\baselineskip}
\end{figure*}

%preemption  (we use negative)
%There is no deliberately perturbation 
%this is different from a covert channel
%novel 
% we observe when we run or we are not running
%covert channel actively cause preemption to 
%IDS


Consider the scenario where you want to attack an embedded real-time system --
parts of autonomous cars, industrial robots, anti-lock braking systems in
modern cars, unmanned aerial vehicles (UAVs), power grid components, the NASA
rovers, implanted medical devices, \etc~(the list is extensive).  These systems
typically have limited memory and processing power, have very regimented
designs (stringent timing constraints for instance) and any unexpected actions
can be quickly thwarted\footnote{Due to the design of such systems, where deadlines
will be missed and the system scheduler might even shut it down.}.  
Therefore, the opportunity to either steal a critical piece
of information or the ability to launch that attack which takes control of the system
is very limited. So, what is a modern-day attacker to do? Be better
informed, of course! This ``information'' can take many forms -- from an
understanding of the design of the system, to knowledge of the critical
components (either software or hardware). The exact knowledge depends on the
type of attack and the target component: \ca say, to steal important
information about when (and where) an on-board camera is used for
reconnaissance or \cb to take control away from the ground operator of a
remotely-controlled vehicle.

The one common underlying theme that pervades real-time systems (and something
that a would-be attacker should definitely gather) is the importance of {\em
timing}\footnote{As we shall see timing plays an all too important a role in
the design and correct operation of real-time systems.}. ``Timing'' includes:
\ci when certain events occurs, \cii how often they occur, and, most
importantly for this paper, \ciii {\em when (and if) they will occur again in the
future}. In fact, a number of critical software components in real-time systems
are designed to be repetitive in terms of timing behavior -- \ie they are
\textit{periodic} in nature. Examples include engine controllers in cars and
aircraft, code that controls industrial and power systems, sensor data
collectors, motor actuators, system heartbeat keepers, \etc~ As we shall see, 
these periodic (and often all important) tasks\footnote{A task in typical 
real-time system corresponds to a process/thread in generic operating systems. 
We use ``task'' and ``process'' interchangeably.} 
present themselves as prime targets for our friendly neighborhood attacker. 

So, how does one attack such systems, especially the periodic (and critical) 
components\footnote{We shall see potential end results of such attacks 
in Section \ref{sec:casestudies}.}? 
\begin{quote}
	\textit{We have discovered the presence of a scheduler-based side-channel 
	that leaks timing information in real-time systems -- in
	particular those with fixed priority tasks}\footnote{In fixed-priority
	systems, all the tasks have priorities, assigned at design time, that
	do not change for the lifetime of the system (see Section
	\ref{sec:model}).}. 
    %\hl{We developed efficient algorithms to leverage this side-channel to extract critical timing information.}
\end{quote}
In fact, the above information leakage can be achieved using an {\em
unprivileged, low-priority task} to reconstruct the precise
timing behavior of the critical (victim) task(s). This provides our attacker
with the ability to {\em precisely predict future execution
instances of the victim task at runtime}! We name the algorithms that exploit this
side-channel attack, ``\ATTCK''.

Figure \ref{fig:paper_overview} presents an overview of the side-channel and
also how the attacker can benefit from the scheduler side-channel-based information (the
right hand side). The left side of the figure shows how a real-time system
consisting of fixed-priority tasks (the boxes at the top) that results in a
schedule (dotted boxes in the middle, with each task being indistinguishable from
the other at runtime) can be analyzed to extract the precise execution points
(the green, upward arrows) of the victim task. The right hand side of the
figure 
%lists how this timing information of the critical task can be used to
shows how this timing information of the critical task can be used to
launch other attacks that either leak more important information (\eg points 
of interest in a UAV's mission) or destabilize the real-time control system 
(\eg either cause it to crash or even prevent a remote operator from controlling it).  
Note that without this precise timing information, an attacker is either
forced to guess when the victim task(s) will execute or launch the attacks at
random points in time -- both of which dilute the efficacy of the attack or
result in early termination of the system (perhaps even before the attack actually succeeds).

The extraction of this run-time timing information is non-trivial. In fact,
Section \ref{sec::discussion} demonstrates why existing techniques are insufficient
for tackling this problem; main reasons include \ca the run-time schedule
depends heavily on the state of the system at startup, initialization variables and
environmental conditions and \cb such real-time systems typically consist of
multiple real-time and non-real-time tasks (other than the victim). Even
precise knowledge of \textit{all} statically-known system parameters is
insufficient to reconstruct the future arrival times of the victim. 
Runtime commands such as $\mathtt{ps}$ or $\mathtt{top}$ cannot provide these ``arrival times'' (\ie when {\em future} instances of the target task will start executing) since
the attacker (who enters the system at an arbitrary point in time and not at
system startup) has no intuition of \textit{when the first instance of each
task in the system started executing}. While a
privileged attacker could target the scheduler of the system and extract the
requisite information, such access typically requires significant effort and/or
resources.  On the other hand, we are able to reconstruct the information with
the same level of precision using an \textit{unprivileged user space
application}.  In fact, all that the attacker's application has to do is keep
track of its own scheduling information! This, coupled with some additional
(easily obtainable) information about the system, can recreate the timing
information with high precision. 

To be more specific, let's say that we want to override the (remote) control of
a rover. In many such systems, a periodic pulse width modulation (PWM) task
drives the steering and throttle. Without knowledge of the precise
points in time when the PWM task updates the motor control values, the
attacker is forced to employ brute force or random strategies to
override the PWM values. These could either end up being ineffective or lead to
the entire system being reset before the attack succeeds (see Section
\ref{sec:casestudies} for more details on this and the next scenario). Armed
with knowledge from \ATTCK, our smart adversary can now override the PWM values
{\em right after} they have been written by the corresponding task --
effectively overriding the actuation commands.

Now consider a different scenario -- that of a reconnaissance
drone who's primary function is to take pictures at certain ``points of
interest''.  Our adversary would, ideally, like to get access to the photographs
and the locations where they were taken. Considering that such images are
typically encrypted and that breaking the encryption in a much harder problem,
we could be satisfied with knowledge of \textit{where} the ``interesting''
photos were taken. An inspection of the cache usage of the image
processing task could provide hints as to when the camera is taking photos of the
interesting points. 
%turned on (or switched
%into a high resolution mode)\footnote{It is quite likely that the camera is not
%always on or even if it is, stays in a low resolution mode most of the time to
%conserve battery power.}. 
If \ATTCK can highlight future times when the image processing task
will execute, we can monitor the latter's cache usage in a fairly precise manner.
%whether it is using the cache at a higher capacity.  
This information, coupled with others (say,  GPS coordinates) leaks
important information about the mission -- \viz ~the points of high interest!
Without the (future) timing information, we will have to launch the
cache-based attack at arbitrary points in time and deal with significant loss of precision
and higher noise in the results. 

Scheduler covert channels, where two processes covertly communicate using the
scheduler, have long been known (\eg~\cite{embeddedsecurity:volp2008,
ghassami2015capacity, embeddedsecurity:son2006}). In contrast, our focus is on
a \textit{side-channel that leaks execution timing behavior (not deliberately!)
of critical, high-priority real-time tasks to say, unprivileged, low-priority
tasks}. We focus on systems with a preemptive,
fixed-priority real-time task scheduler~\cite{Buttazzo:1997:HRC,LiuLayland1973}
since they are the most common class of real-time systems deployed in practice
today~\cite{Liu:2000:RTS}. It is important for our attacker to \textit{stay
within the strict execution time budgets} alloted to the unprivileged task
(that we intend to hijack for our purposes) -- especially during the phases
when it is trying to observe and reconstruct the victim's timing behavior.
Failing this requirement will likely cause other critical real-time
functionality to fail or trigger a watchdog timeout that resets the system,
leading to premature ejection of the attacker\footnote{Most real-time systems do not have an intrusion detection system (IDS).
Yet, violating the real-time guarantees 
%and causing real-time tasks to miss their deadlines 
would be detected by the scheduler or an existing system error monitor.}.  This
property is crucial during the `reconnaissance' phase of what come to be known as
advanced persistent threat (APT) attacks~\cite{tankard2011advanced,
virvilis2013big}.  For instance, it has been reported that attackers had
penetrated and stayed resident undetected in the system for {\em months} before
they initiated the actual attack in the case of
Stuxnet~\cite{stuxnet:symantecdossier11}.  Once they had enough information
about the precise nature of the system, they were able to craft effective
attacks that were tailored to that particular system.

The \ATTCKNF algorithms are implemented on both a simulator and real hardware platforms 
running Real-Time Linux and FreeRTOS operating systems (for the two attack 
case studies). We evaluate the
performance and scalability of \ATTCKNF in Section~\ref{sec::eval}, along with
a design space exploration (on the simulator). The results show that our methods are
effective at reconstructing schedule information and provide valuable
information for later attacks to better accomplish their attack goals.  To
summarize, the main contributions are: 
%\vspace{-0.5\baselineskip}
\begin{tight_enumerate}
\item Novel scheduler side-channel attack algorithms that can accurately
reconstruct the execution timing behaviors of critical real-time
tasks in real-time systems (without
requiring privileged access) [Section~\ref{sec::approach}]

\item Analyses and metrics to measure the accuracy in predicting the execution
and timing properties of the victim tasks [Section~\ref{sec::analysis}
and Section~\ref{sec::eval}].
\end{tight_enumerate}



\begin{comment}
%Commented by Sibin

\hl{New Intro.}
Autonomous control systems such as self-driving cars, medicine/vaccine delivery drones, space rovers (\eg NASA's Opportunity and Spirit), industrial robots, autonomous tractors and military surveillance unmanned aerial vehicles (UAV), play a vital role in shaping today's technological evolution from everyday living to space exploration.
In such systems, tasks\footnote{A task in typical real-time systems corresponds to a process/thread in generic operating systems. In this paper, we will use ``task'' and ``process'' interchangeably.} delivering critical functionality rely on an operating system (typically a real-time operating system or an operating system that supports a real-time scheduling policy) to fulfill their timing requirements (\eg the task must complete within a predefined time limit). Oftentimes, these tasks (\eg system heartbeat keepers, PID control processes, sensor data collectors, motor actuators) are designed as real-time tasks and executed in a periodic fashion to guarantee responsiveness.
However, such periodicity turns out to leak valuable timing information and poses threats to the entire systems.
As we point out in this paper, a scheduler side-channel that exploits the periodic nature exists in a preemptive, fixed-priority real-time task scheduler (the most common class of schedulers in real-time autonomous control systems).
We show that a smart adversary can use {\em an unprivileged, low-priority task} to exploit such a scheduler side-channel to recover execution behaviors of the targeted real-time tasks (that we call ``victim'' tasks) {\em at runtime}.
The outcome is the precise inference of the victim task's future execution points in time (this paper introduces attack algorithms that achieve exactly that). This type of reconnaissance techniques and the obtained information are particularly useful in the case of advanced persistent threat (APT) attacks~\cite{tankard2011advanced, virvilis2013big}.

In Section~\ref{sec:casestudies} we show the importance of such task timing information in two attack cases where reconnaissance attacks are necessary for achieving their major attack goals \hl{without risking detection}.
%
In one case, the adversary intends to override the control of an autonomous rover by interleaving the pulse-width modulation (PWM) signals that drive steering and throttle. The PWM signals are updated periodically by a real-time task (the victim task) by design. Without knowing the exact time points when the victim task is updating the PWM signals, the attacker can either issue the PWM updates at arbitrary time points which is ineffective or can employ a brute force strategy with a very high overhead which can influence other critical real-time tasks and crash the system. On the other hand, with a reconnaissance attack to obtain timing information of the victim task in advance, the attacker may precisely issue an PWM update right after the original update to effectively override the output.
%

In another case on a surveillance UAV, the adversary intends to monitor the execution behaviors of a real-time task (the victim task) to further infer the UAV's mission targets.
A cache-time side-channel attack is employed in this case in an attempt to gauge the victim task's memory usage. 
Again, without a reconnaissance attack for learning the victim task's execution time points, the attacker can only launch the cache-timing side-channel attacks at arbitrary instants. The outcome is mixed memory usage of both the victim task and other irrelevant tasks. 
In contrast, with the timing information an attacker can launch the cache-timing side-channel attacks only around the instants when the victim task is active. 
As we will see in the case study, execution behaviors of the victim task can be observed and further valuable information about the UAV's mission can be identified.
%In both cases, knowing exactly when the victim task is scheduled helps 
\end{comment}
% Commented by Sibin


\begin{comment}
%An unmanned aerial vehicle (UAV) executing a surveillance mission exemplifies the exploitation of such vulnerability.
%To exemplify the exploitation of the schedule information, %of this real-time scheduler vulnerability, 
For example, let us consider an unmanned aerial vehicle (UAV) executing a surveillance mission.
The UAV runs a real-time operating system where multiple real-time tasks are used for navigation, communication and surveillance, \etc~
The UAV's objective is to fly over some territory and capture high-resolution images when it reaches locations of interest.
Assume that adversary has a user-space task in the system (for example, through a supply chain vulnerability). Here, the attacker's goal is not to crash the UAV.
Rather, %the attacker wants to sit in the UAV and quietly learn what locations it is interested in.
the attacker wants to {\em stealthily} learn the locations of high-interest targets (where the surveillance camera is switched to a high-resolution image mode).
%Here, we mainly focus on the attacker's objective of learning locations of high-interest targets where the surveillance camera on the UAV is enabled.
%This can be done by monitoring the memory usage of the task that handles the pictures taken by the on-system surveillance camera.
%This can be done by monitoring the behavior (\eg memory usage) of the periodic real-time task that handles the pictures taken by the on-system surveillance camera (\ie higher cache usage indicates that a high-resolution image is being processed).
This can be done by monitoring the memory usage behavior of the $30Hz$ real-time task that handles the images captured by the surveillance camera. 
In particular, a cache-timing side-channel attack against such a victim task can be used to gauge its memory usage.
A higher memory usage would indicate that a high-resolution image is being processed while a relatively lower memory usage shows that the operation of surveillance is inactive or on standby.
However, as there are many tasks running in the same system, 
%it is infeasible 
without knowing when the victim task is scheduled to run, a random sampling of the cache will result in noisy -- often useless, data.
By exploiting the extracted schedule information,
%aforementioned scheduler vulnerability and reconstructing the schedule for the victim task, 
the attacker can precisely execute prime and probe attacks \cite{osvik2006cache, page2002theoretical} before and after the victim task is executed. 
This attack is implemented and discussed in Section~\ref{sec:cache_timing_attack}. 
\end{comment}

\begin{comment}
%Commented by Sibin
While the scheduler side-channel presented in this paper exists in most autonomous control systems with real-time tasks, it is not trivial to learn and extract the exact times that the victim tasks are scheduled at {\em runtime}. 
In Section~{\ref{sec::dft}}, we show that existing techniques cannot trivially handle this problem.
It is because \ci the actual schedule depends on the system start-up and initialization and other environmental conditions and \cii 
there may be multiple real-time and non-real-time tasks other than the victim task in the system that contribute to the uncertainty of the runtime schedule.  In other words, without considering runtime variation, even knowledge of all the predefined parameters (\ie periods, deadlines and the worst-case execution times) of all tasks alone is insufficient to reconstruct the actual, runtime schedule. 
%\hl{While a privileged attacker might be able to extract the schedule directly from the scheduler, here we show that even an unprivileged attacker is able to learn the schedule of a high-priority, critical real-time victim using only a low-priority, user-space task by leveraging the scheduler side-channel.}
While a privileged attacker might be able to extract the schedule directly from the scheduler, in this paper we show that even an unprivileged attacker is able to learn the schedule of the victim task by using the proposed attack algorithms via the scheduler side-channel. %a high-priority, critical real-time victim by using the proposed scheduler side-channel attack algorithms.}

%Further, oftentimes the attacker/intruder can only obtain user privileges and hence is restricted in attack capabilities; \civ differing from a scheduler covert channel in which the adversary deliberately perturbs the schedule to convey information~\cite{embeddedsecurity:volp2008}, our goal is to stealthily gather and extract information.
%Therefore, it is crucial for the attacker to not perturb the strict timing properties of the system, especially for the real-time tasks. 
%Failing this will likely lead to early detection of the attack code, cause critical real-time functionality to fail or even trigger a watchdog timeout. 
%\civ as the goal is to stealthily gather and extract information, it is crucial for the attacker to not perturb the strict timing properties of the system, especially for the real-time tasks. Failing this will likely lead to early detection of the attack code or causing critical real-time functionality to fail. 
%As a result, an attack algorithm like the one presented in this paper is needed.
%that does reconnaissance is needed. %that learns the schedule information is needed. 
%

% While most autonomous control systems with real-time tasks are vulnerable to the scheduler side-channel attacks presented in this paper, it is not trivial to learn and extract the exact times that the victim tasks are scheduled from the {\em runtime schedule}.
% It is because \ci as we mentioned in the above demonstrative attack, there are other real-time tasks (either sporadic or periodic) in the system that contribute to the  uncertainty of runtime schedule ; \cii the actual schedule depends on the system start-up and initialization and other environmental conditions. In other words, to the attacker, even knowing all the predefined parameters (\ie periods, deadlines and WCET) about the tasks is insufficient to reconstruct the actual schedule; \ciii oftentimes the attacker/intruder can only obtain user privileges and hence is restricted in attack capabilities; 
% \civ differing from a scheduler covert channel in which the adversary deliberately perturbs the schedule to convey information~\cite{embeddedsecurity:volp2008}, our goal is to stealthily gather and extract information.
% Therefore, it is crucial for the attacker to not perturb the strict timing properties of the system, especially for the real-time tasks. 
% Failing this will likely lead to early detection of the attack code, cause critical real-time functionality to fail or even trigger a watchdog timeout. 
%
% %\civ as the goal is to stealthily gather and extract information, it is crucial for the attacker to not perturb the strict timing properties of the system, especially for the real-time tasks. Failing this will likely lead to early detection of the attack code or causing critical real-time functionality to fail. 

In this paper, we present novel attack algorithms, named ``\ATTCK'', that exploit the scheduler side-channel in real-time autonomous control systems.
We show that the scheduler side-channel can be exploited by an unprivileged, compromised low-priority task (that can be either a real-time or a non-real-time task) by simply observing its own execution intervals (\ie when the low-priority task itself is running and when it isn't -- which does not require any privilege in most operating systems).
The \ATTCKNF algorithms reconstruct initial execution offsets and infer future execution time points of critical, high-priority real-time task(s) using observations from a malicious low-priority task, which enables adversaries to launch more devastating attacks at those future execution points of critical victim tasks. It is important to note that scheduler covert channels where two processes covertly communicate using the scheduler have long been known (\eg~\cite{embeddedsecurity:volp2008, ghassami2015capacity, embeddedsecurity:son2006}). In contrast, our focus is on a side-channel that leaks execution timing behavior of critical, high-priority real-time tasks to any unprivileged, low-priority tasks.
%The periodicity of the real-time tasks turns out to {\em leak valuable execution timing behaviors from critical, high priority real-time task(s) to an unprivileged low priority task via the scheduler side-channel} and poses a threat to the systems when it comes down to safety and security.
\end{comment}
% Commented by Sibin

\begin{comment}
Real-time tasks are usually constrained by their predefined periods, deadlines, the worst-case execution times (WCET) and real-time scheduling algorithms (\eg fixed-priority preemptive scheduling, earliest deadline first scheduling~\cite{LiuLayland1973}).
These real-time constraints help system designers analyze the system as a whole and ensure that all safety guarantees are met (\eg no real-time tasks will miss their deadlines).
As a result, the system schedule (even a mix of both real-time and non-real-time tasks) becomes highly predicable.
This predictability, though favorable for the system analysis and safety, is a double-edged sword. % -- it creates side-channels in the real-time task scheduler.
A smart attacker can exploit the scheduler side-channels and the predictable nature of the system schedule to recover execution behaviors of the targeted tasks (that we call ``victim'' tasks) {\em at runtime} (our attack algorithms achieve exactly that). 
Knowing the precise schedule of the victim real-time tasks enables the attacker to pinpoint their future execution patterns.
%that can create attacker's interest to the fullest extent when launching a greater attack later.
%and launch greater attacks to gain even more information or cause the damage to the fullest extent.
The adversary can then launch more devastating attacks at those future execution points of victim tasks.
%In this paper, we present novel scheduler side-channel attack algorithms that take advantage of the predicable nature of the real-time tasks to gather and extract information about their precise timing behavior.
\end{comment}


\begin{comment}
%Commented by Sibin

%Specifically, we present novel scheduler side-channel attack algorithms, named ``\ATTCK''. %for reconnaissance against real-time tasks in autonomous control systems. 
In this paper, we focus on autonomous control systems with a preemptive, fixed-priority real-time task scheduler~\cite{Buttazzo:1997:HRC,LiuLayland1973} since they are the most common class of real-time systems deployed in practice today~\cite{Liu:2000:RTS}. 
%Also, this class of systems (rather, the preemptive, fixed-priority scheduling algorithms) is most vulnerable to attacks since they are very {\em predictable} (by design). 
%\hl{However, predictability of such systems also means that any deviations in execution time behavior can easily be detected.}
%The \ATTCKNF algorithms exploit the nature of preemptions in fixed-priority, preemptive real-time schedulers that allow high priority tasks to preempt low priority tasks.
%With the \ATTCKNF algorithms, we are able to reconstruct the precise execution schedule of a periodic real-time victim task in the system by leveraging a compromised lower-priority user-space task. 
The \ATTCKNF algorithms can carry out the attack while \emph{staying within the execution time limits} of the compromised task.
%to reduce chances of detection and \hl{as such are particularly suitable for conducting reconnaissance and gathering information before launching more targeted attacks.}
It is particularly crucial for the attacker to not perturb the strict timing properties of the real-time autonomous control system, especially in the stage of reconstructing the information. %for the real-time tasks. 
Failing this will likely cause other critical real-time functionality to fail or trigger a watchdog timeout that resets the system, leading to pre-mature detection of the attacker\footnote{Most real-time autonomous control systems do not have an intrusion detection system (IDS). Yet, violating the real-time guarantees 
%and causing real-time tasks to miss their deadlines 
would be detected by the scheduler or an existing system error monitor.}.
%
%\ATTCKNF algorithms can carry out the attack while \emph{staying within the execution time limits} of the compromised task to reduce chances of detection and \hl{as such are particularly suitable for conducting reconnaissance and gathering information before launching more targeted attacks.}
%
%In general, reconnaissance is usually a stepping stone to more complex and powerful attacks~\cite{rowe2007thwarting, durdaugi2010ipv4} and is part of the intelligence gathering stage of such attacks~\cite{stolfo2004worm}. 
%
This property is essential in the reconnaissance phase in APT attacks.
For instance, it has been reported that attackers had penetrated and stayed resident undetected in the system for {\em months} before they initiated the actual attack in the case of Stuxnet~\cite{stuxnet:symantecdossier11}. 
Once they had enough information about the precise nature of the system, they were able to craft effective attacks that were tailored to that particular system. %-- thus causing the most amount of damage. Hence, {\em reconnaissance} is a critical phase for attacks on such systems.
%\hl{The proposed attack algorithms are particularly suitable for conducting reconnaissance and gathering information before launching more targeted attacks.}
%Section~\ref{sec::analysis} explores the parameters for this property.
%Note that the focus of this paper is not on compromising the task but showing how such an unprivileged (compromised) task can infer the precise details of when the target/victim task executes by observing its own execution behavior. 

The \ATTCKNF algorithms are implemented on both a simulator (for performance evaluation) and real hardware platforms running Real-Time Linux %(running on a real custom remote rover) 
and FreeRTOS %(running on a UAV platform) 
operating systems (for the two attack case studies).
%
%\hl{Two attack cases are studied in Section~{\ref{sec:casestudies}} to show} how extracted real-time task schedule information can help  stage other, more debilitating attacks.
%
%Two attacks are demonstrated on the real hardware platforms to show that utilizing information gained from \ATTCKNF can help stage other, more debilitating attacks in Section~\ref{sec::eval_platform}. 
%Specifically we demonstrate how extracted schedule information can help \ci reduce attack overhead (in a control signal interleaving attack on a custom rover) and \cii increase attack precision (in a cache-timing side-channel attack on a hardware-in-the-loop UAV platform).
We evaluate the performance and scalability of \ATTCKNF in Section~\ref{sec::eval}, along with a design space exploration.
The evaluation results show that our methods are effective at reconstructing schedule information and provide valuable information for later attacks to better accomplish their attack goals. 
%
% \begin{figure}[h] %\vspace{-1\baselineskip} \centering
% %[width=0.85\columnwidth]
% \includegraphics[width=0.85\columnwidth]{Figures/schedule_based_brief}
% %\vspace{-0.5\baselineskip} \caption{Illustration of the schedule
% timing-based side-channel.} \label{fig:schedule_based_brief}
% %\vspace{-0.5\baselineskip} \end{figure}
%
Figure~\ref{fig:paper_overview} shows an overview of the paper. %proposed attack algorithms and scope of this paper.
The left side of the figure depicts the high-level concept of the proposed \ATTCKNF attack and the right side illustrates possible attacks enabled by \ATTCKNF. 
To summarize, the main contributions are: 
%\vspace{-0.5\baselineskip}
\begin{tight_enumerate}
	%\item Novel reconnaissance attack algorithms (based on a novel scheduler side-channel) that can accurately reconstruct the	timing behavior of critical real-time tasks in real-time autonomous control systems. [Section~\ref{sec::approach}]
    \item Novel scheduler side-channel attack algorithms that can accurately reconstruct the execution timing behaviors of critical real-time tasks in real-time autonomous control systems (without requiring privileged access). [Section~\ref{sec::approach}]
	%\item The ability to carry out such a reconnaissance attack while minimizing the risk of detection. [Section~\ref{sec::analysis}]
	\item Analyses and metrics to measure the accuracy in predicting the execution and timing properties of the victim tasks. [Section~\ref{sec::analysis} and Section~\ref{sec::eval}]
    %\item Demonstration of the feasibility and value of reconnaissance attack with two attack scenarios on real hardware platforms running the FreeRTOS (an UAV platform) and Real-Time Linux (a real custom quadcopter and a remote rover) operating systems. [Sections~\ref{sec::eval_platform}]
	%\item Anything else?
% \item We define \emph{observability}, a term for describing the property of
		% observation in the schedule-based side-channel in general.
		% \item We propose a generalized \emph{observe-converge-expand}
		% model for the attacks based on the schedule-based
		% side-channel.  \item We introduce algorithms that implement
		% \emph{observe-converge}. An observation lower bound and an
		% upper bound are derived in such an implementation.% by a
		% mathematical proof.
% %\item We introduce the \emph{schedule ladder diagram}, a new utility for
		% analyzing task schedule.
\end{tight_enumerate}

%\vspace{-0.5\baselineskip}

%The rest of the paper is outlined as follows: \emph{Section~\ref{sec::model}}
%introduces the system configurations and
%knowledge 
%requirements for adversaries to utilize the schedule-based side-channel.
% \emph{Section~\ref{sec::schedule_attack_overview}} defines the schedule-based
% side channel and gives an insight into the scope of the attack introduced in
% this paper.  %before theorem bases are given.
% \emph{Section~\ref{sec::observe_bi}} elaborates how execution intervals can
% be observed by the adversary.  \emph{Section~\ref{sec::extract_and_infer}}
% discusses how the victim task's executions can be extracted from the observed
% execution intervals.  \emph{Section~\ref{sec::bound_and_observability}}
% derives an observation lower bound and an upper bound for the adversary to
% sufficiently extract useful information against the victim task. The way to
% determine the observability of the observer task is also detailed in this
% section.% for inferring the victim task's arrivals and gives the theorem to
% determine the observability of the observer task.

%TBD The evaluation is given in \emph{Section~\ref{sec::eval}}.

\end{comment}
% Commented by Sibin



==> Sections/intro_NDSS19_CY.tex <==
\section{Introduction}
\label{sec::intro}

\begin{figure*}[t]
%\vspace{-\baselineskip}
\centering
\includegraphics[width=0.95\textwidth]{Figures/paper_overview}
%\vspace{-0.7\baselineskip}
\caption{Overview of this paper. We focus on how an unprivileged, low-priority task can utilize the \ATTCKNF algorithms to infer the execution behaviors of critical, high-priority real-time task(s). %the precise details of the victim task's schedule with an unprivileged task.
Two advanced attacks enabled by \ATTCKNF are shown in this paper to demonstrate possible use cases of the extracted side-channel information. %damage from using the information provided by the \ATTCKNF algorithms.
}
\label{fig:paper_overview}
\vspace{-1.5\baselineskip}
\end{figure*}

%preemption  (we use negative)
%There is no deliberately perturbation 
%this is different from a covert channel
%novel 
% we observe when we run or we are not running
%covert channel actively cause preemption to 
%IDS

%\hl{Add something about APT.}
Real-time systems such as self-driving cars, medicine/vaccine delivery drones, space rovers (\eg NASA's Opportunity and Spirit), industrial robots, autonomous tractors and military surveillance unmanned aerial vehicles (UAV), play a vital role in shaping today's technological evolution from everyday living to space exploration.
In such systems, tasks\footnote{A task in typical real-time systems corresponds to a process/thread in generic operating systems. In this paper, we will use ``task'' and ``process'' interchangeably.} delivering critical functionality rely on an operating system (typically a real-time operating system or an operating system that supports a real-time scheduling policy) to fulfill their timing requirements (\eg the task must complete within a predefined time limit). Oftentimes, these tasks (\eg system heartbeat keepers, PID control processes, sensor data collectors, motor actuators) are designed as real-time tasks and executed in a periodic fashion to guarantee responsiveness.
However, as we point out in this paper, a scheduler side-channel exists in a preemptive, fixed-priority real-time task scheduler (the most common class of schedulers in real-time autonomous control systems).
This side-channel can leak valuable timing behaviors of critical, high-priority real-time task(s) to unprivileged low-priority tasks (that can be either a real-time or a non-real-time task).
We show that this side-channel can be exploited by %an unprivileged 
a malicious/compromised low-priority task by simply observing its own execution intervals (\ie when the low-priority task itself is running and when it isn't).
In particular, we present novel attack algorithms, named ``\ATTCK'', that exploit the scheduler side-channel in real-time autonomous control systems. It is important to note that scheduler covert channels where two processes covertly communicate using the scheduler have long been known (\eg~\cite{embeddedsecurity:volp2008, ghassami2015capacity, embeddedsecurity:son2006}). In contrast, our focus is on a side-channel that leaks execution timing behavior of critical, high-priority real-time tasks to any unprivileged, low-priority tasks.
%The periodicity of the real-time tasks turns out to {\em leak valuable execution timing behaviors from critical, high priority real-time task(s) to an unprivileged low priority task via the scheduler side-channel} and poses a threat to the systems when it comes down to safety and security.

Real-time tasks are usually constrained by their predefined periods, deadlines, the worst-case execution times (WCET) and real-time scheduling algorithms (\eg fixed-priority preemptive scheduling, earliest deadline first scheduling~\cite{LiuLayland1973}).
These real-time constraints help system designers analyze the system as a whole and ensure that all safety guarantees are met (\eg no real-time tasks will miss their deadlines).
As a result, the system schedule (even a mix of both real-time and non-real-time tasks) becomes highly predicable.
This predictability, though favorable for the system analysis and safety, is a double-edged sword. % -- it creates side-channels in the real-time task scheduler.
A smart attacker can exploit the scheduler side-channels and the predictable nature of the system schedule to recover execution behaviors of the targeted tasks (that we call ``victim'' tasks) {\em at runtime} (our attack algorithms achieve exactly that). 
Knowing the precise schedule of the victim real-time tasks enables the attacker to pinpoint their future execution patterns.
%that can create attacker's interest to the fullest extent when launching a greater attack later.
%and launch greater attacks to gain even more information or cause the damage to the fullest extent.
The adversary can then launch more devastating attacks at those future execution points of victim tasks.
%In this paper, we present novel scheduler side-channel attack algorithms that take advantage of the predicable nature of the real-time tasks to gather and extract information about their precise timing behavior.


%An unmanned aerial vehicle (UAV) executing a surveillance mission exemplifies the exploitation of such vulnerability.
%To exemplify the exploitation of the schedule information, %of this real-time scheduler vulnerability, 
For example, let us consider an unmanned aerial vehicle (UAV) executing a surveillance mission.
The UAV runs a real-time operating system where multiple real-time tasks are used for navigation, communication and surveillance, \etc~
The UAV's objective is to fly over some territory and capture high-resolution images when it reaches locations of interest.
Assume that adversary has a user-space task in the system (for example, through a supply chain vulnerability). Here, the attacker's goal is not to crash the UAV.
Rather, %the attacker wants to sit in the UAV and quietly learn what locations it is interested in.
the attacker wants to {\em stealthily} learn the locations of high-interest targets (where the surveillance camera is switched to a high-resolution image mode).
%Here, we mainly focus on the attacker's objective of learning locations of high-interest targets where the surveillance camera on the UAV is enabled.
%This can be done by monitoring the memory usage of the task that handles the pictures taken by the on-system surveillance camera.
%This can be done by monitoring the behavior (\eg memory usage) of the periodic real-time task that handles the pictures taken by the on-system surveillance camera (\ie higher cache usage indicates that a high-resolution image is being processed).
This can be done by monitoring the memory usage behavior of the $30Hz$ real-time task that handles the images captured by the surveillance camera. 
In particular, a cache-timing side-channel attack against such a victim task can be used to gauge its memory usage.
A higher memory usage would indicate that a high-resolution image is being processed while a relatively lower memory usage shows that the operation of surveillance is inactive or on standby.
However, as there are many tasks running in the same system, 
%it is infeasible 
without knowing when the victim task is scheduled to run, a random sampling of the cache will result in noisy -- often useless, data.
By exploiting the extracted schedule information,
%aforementioned scheduler vulnerability and reconstructing the schedule for the victim task, 
the attacker can precisely execute prime and probe attacks \cite{osvik2006cache, page2002theoretical} before and after the victim task is executed. 
This attack is implemented and discussed in Section~\ref{sec:cache_timing_attack}. 
%\todo{RBB:not sure what the goal of the following paragraph is. justifying why the problem is not trivial? See if the changes look OK. Saved the old copy. \\CY:Thanks, I checked and revised.}

While most autonomous control systems with real-time tasks are vulnerable to the scheduler side-channel attacks presented in this paper, it is not trivial to learn and extract the exact times that the victim tasks are scheduled at {\em runtime}. 
In Section~{\ref{sec::discussion}}, we show that other existing analysis techniques cannot trivially handle this problem.
It is because \ci the actual schedule depends on the system start-up and initialization and other environmental conditions and \cii 
there may be multiple real-time and non-real-time tasks other than the victim task in the system that contribute to the uncertainty of the runtime schedule.  In other words, even knowledge of all the predefined parameters (\ie periods, deadlines and WCET) of all tasks alone is insufficient to reconstruct the actual schedule. 
%\hl{While a privileged attacker might be able to extract the schedule directly from the scheduler, here we show that even an unprivileged attacker is able to learn the schedule of a high-priority, critical real-time victim using only a low-priority, user-space task by leveraging the scheduler side-channel.}
While a privileged attacker might be able to extract the schedule directly from the scheduler, here we show that even an unprivileged attacker is able to learn the schedule of the victim task by using the proposed attack algorithms. %a high-priority, critical real-time victim by using the proposed scheduler side-channel attack algorithms.}

%Further, oftentimes the attacker/intruder can only obtain user privileges and hence is restricted in attack capabilities; \civ differing from a scheduler covert channel in which the adversary deliberately perturbs the schedule to convey information~\cite{embeddedsecurity:volp2008}, our goal is to stealthily gather and extract information.
%Therefore, it is crucial for the attacker to not perturb the strict timing properties of the system, especially for the real-time tasks. 
%Failing this will likely lead to early detection of the attack code, cause critical real-time functionality to fail or even trigger a watchdog timeout. 
%\civ as the goal is to stealthily gather and extract information, it is crucial for the attacker to not perturb the strict timing properties of the system, especially for the real-time tasks. Failing this will likely lead to early detection of the attack code or causing critical real-time functionality to fail. 
%As a result, an attack algorithm like the one presented in this paper is needed.
%that does reconnaissance is needed. %that learns the schedule information is needed. 
%

% While most autonomous control systems with real-time tasks are vulnerable to the scheduler side-channel attacks presented in this paper, it is not trivial to learn and extract the exact times that the victim tasks are scheduled from the {\em runtime schedule}.
% It is because \ci as we mentioned in the above demonstrative attack, there are other real-time tasks (either sporadic or periodic) in the system that contribute to the  uncertainty of runtime schedule ; \cii the actual schedule depends on the system start-up and initialization and other environmental conditions. In other words, to the attacker, even knowing all the predefined parameters (\ie periods, deadlines and WCET) about the tasks is insufficient to reconstruct the actual schedule; \ciii oftentimes the attacker/intruder can only obtain user privileges and hence is restricted in attack capabilities; 
% \civ differing from a scheduler covert channel in which the adversary deliberately perturbs the schedule to convey information~\cite{embeddedsecurity:volp2008}, our goal is to stealthily gather and extract information.
% Therefore, it is crucial for the attacker to not perturb the strict timing properties of the system, especially for the real-time tasks. 
% Failing this will likely lead to early detection of the attack code, cause critical real-time functionality to fail or even trigger a watchdog timeout. 

% %\civ as the goal is to stealthily gather and extract information, it is crucial for the attacker to not perturb the strict timing properties of the system, especially for the real-time tasks. Failing this will likely lead to early detection of the attack code or causing critical real-time functionality to fail. 


% As a result, an attack algorithm like the one presented in this paper is needed.
% %that does reconnaissance is needed. %that learns the schedule information is needed. 
%

%Specifically, we present novel scheduler side-channel attack algorithms, named ``\ATTCK''. %for reconnaissance against real-time tasks in autonomous control systems. 
In this paper, we focus on autonomous control systems with a preemptive, fixed-priority real-time task scheduler~\cite{Buttazzo:1997:HRC,LiuLayland1973} since they are the most common class of real-time systems deployed in practice today~\cite{Liu:2000:RTS}. 
Also, this class of systems (rather, the preemptive, fixed-priority scheduling algorithms) is most vulnerable to attacks since they are very {\em predictable} (by design). %\hl{However, predictability of such systems also means that any deviations in execution time behavior can easily be detected.}
%The \ATTCKNF algorithms exploit the nature of preemptions in fixed-priority, preemptive real-time schedulers that allow high priority tasks to preempt low priority tasks.
With the \ATTCKNF algorithms, we are able to reconstruct the precise execution schedule of a periodic real-time victim task in the system by leveraging a compromised lower-priority user-space task. 
The \ATTCKNF algorithms can carry out the attack while \emph{staying within the execution time limits} of the compromised task.
%to reduce chances of detection and \hl{as such are particularly suitable for conducting reconnaissance and gathering information before launching more targeted attacks.}
It is particularly crucial for the attacker to not perturb the strict timing properties of the real-time autonomous control system, especially in the stage of reconstructing the information. %for the real-time tasks. 
Failing this will likely cause critical real-time functionality to fail or trigger a watchdog timeout that resets the system, leading to pre-mature detection of the attacker\footnote{Most real-time autonomous control systems do not have an intrusion detection system (IDS). Yet, violating the real-time guarantees 
%and causing real-time tasks to miss their deadlines 
would be detected by the scheduler or any existing system error monitor.}.
%
%\ATTCKNF algorithms can carry out the attack while \emph{staying within the execution time limits} of the compromised task to reduce chances of detection and \hl{as such are particularly suitable for conducting reconnaissance and gathering information before launching more targeted attacks.}
%
%In general, reconnaissance is usually a stepping stone to more complex and powerful attacks~\cite{rowe2007thwarting, durdaugi2010ipv4} and is part of the intelligence gathering stage of such attacks~\cite{stolfo2004worm}. 
%
It has been reported that attackers had penetrated and stayed resident undetected in the system for {\em months} before they initiated the actual attack in the case of Stuxnet~\cite{stuxnet:symantecdossier11}. 
Once they had enough information about the precise nature of the system, they were able to craft effective attacks that were tailored to that particular system. %-- thus causing the most amount of damage. Hence, {\em reconnaissance} is a critical phase for attacks on such systems.
%\hl{The proposed attack algorithms are particularly suitable for conducting reconnaissance and gathering information before launching more targeted attacks.}
%Section~\ref{sec::analysis} explores the parameters for this property.
%Note that the focus of this paper is not on compromising the task but showing how such an unprivileged (compromised) task can infer the precise details of when the target/victim task executes by observing its own execution behavior. 

The \ATTCKNF algorithms are implemented and evaluated on both a simulator and real hardware platforms running Real-Time Linux %(running on a real custom remote rover) 
and FreeRTOS %(running on a UAV platform) 
operating systems.
%
Two attack cases are studied in Section~{\ref{sec:casestudies}} to show how extracted real-time task schedule information can help  stage other, more debilitating attacks.
%
%Two attacks are demonstrated on the real hardware platforms to show that utilizing information gained from \ATTCKNF can help stage other, more debilitating attacks in Section~\ref{sec::eval_platform}. 
%Specifically we demonstrate how extracted schedule information can help \ci reduce attack overhead (in a control signal interleaving attack on a custom rover) and \cii increase attack precision (in a cache-timing side-channel attack on a hardware-in-the-loop UAV platform).
We also evaluate the performance and scalability of \ATTCKNF in Section~\ref{sec::eval}, along with a design space exploration.
The evaluation results show that our methods are effective at reconstructing schedule information and provide valuable information for later attacks to better accomplish their attack goals. 
%
%Note that, while two demonstrative attacks are shown in this paper, the use of the extracted schedule information is not limited to these cases. 

%
% \begin{figure}[h] %\vspace{-1\baselineskip} \centering
% %[width=0.85\columnwidth]
% \includegraphics[width=0.85\columnwidth]{Figures/schedule_based_brief}
% %\vspace{-0.5\baselineskip} \caption{Illustration of the schedule
% timing-based side-channel.} \label{fig:schedule_based_brief}
% %\vspace{-0.5\baselineskip} \end{figure}
%
Figure~\ref{fig:paper_overview} shows an overview of the paper. %proposed attack algorithms and scope of this paper.
The left side of the figure depicts the high-level concept of the proposed \ATTCKNF attack and the right side illustrates possible attacks enabled by \ATTCKNF. 
To summarize, the main contributions are: 
%\vspace{-0.5\baselineskip}
\begin{tight_enumerate}
	%\item Novel reconnaissance attack algorithms (based on a novel scheduler side-channel) that can accurately reconstruct the	timing behavior of critical real-time tasks in real-time autonomous control systems. [Section~\ref{sec::approach}]
    \item Novel scheduler side-channel attack algorithms that can accurately reconstruct the execution timing behaviors of critical real-time tasks in real-time autonomous control systems (without privileged access). [Section~\ref{sec::approach}]
	%\item The ability to carry out such a reconnaissance attack while minimizing the risk of detection. [Section~\ref{sec::analysis}]
	\item Analyses and metrics to measure the accuracy in predicting the execution and timing properties of the victim tasks. [Section~\ref{sec::analysis} and Section~\ref{sec::eval}]
    %\item Demonstration of the feasibility and value of reconnaissance attack with two attack scenarios on real hardware platforms running the FreeRTOS (an UAV platform) and Real-Time Linux (a real custom quadcopter and a remote rover) operating systems. [Sections~\ref{sec::eval_platform}]
	%\item Anything else?
% \item We define \emph{observability}, a term for describing the property of
		% observation in the schedule-based side-channel in general.
		% \item We propose a generalized \emph{observe-converge-expand}
		% model for the attacks based on the schedule-based
		% side-channel.  \item We introduce algorithms that implement
		% \emph{observe-converge}. An observation lower bound and an
		% upper bound are derived in such an implementation.% by a
		% mathematical proof.
% %\item We introduce the \emph{schedule ladder diagram}, a new utility for
		% analyzing task schedule.
\end{tight_enumerate}

%\vspace{-0.5\baselineskip}

%The rest of the paper is outlined as follows: \emph{Section~\ref{sec::model}}
%introduces the system configurations and
%knowledge 
%requirements for adversaries to utilize the schedule-based side-channel.
% \emph{Section~\ref{sec::schedule_attack_overview}} defines the schedule-based
% side channel and gives an insight into the scope of the attack introduced in
% this paper.  %before theorem bases are given.
% \emph{Section~\ref{sec::observe_bi}} elaborates how execution intervals can
% be observed by the adversary.  \emph{Section~\ref{sec::extract_and_infer}}
% discusses how the victim task's executions can be extracted from the observed
% execution intervals.  \emph{Section~\ref{sec::bound_and_observability}}
% derives an observation lower bound and an upper bound for the adversary to
% sufficiently extract useful information against the victim task. The way to
% determine the observability of the observer task is also detailed in this
% section.% for inferring the victim task's arrivals and gives the theorem to
% determine the observability of the observer task.

%TBD The evaluation is given in \emph{Section~\ref{sec::eval}}.




==> Sections/intro_RTAS19_CY.tex <==
\section{Introduction}
\label{sec::intro}


\begin{figure*}[t]
%\vspace{-\baselineskip}
\centering
\includegraphics[width=0.95\textwidth]{Figures/paper_overview}
%\vspace{-0.7\baselineskip}
\caption{Overview of this paper. We focus on how an unprivileged, low-priority task can utilize the \ATTCKNF algorithms to infer the execution behaviors of critical, high-priority real-time task(s). %the precise details of the victim task's schedule with an unprivileged task.
Two advanced attacks enabled by \ATTCKNF are shown in this paper to demonstrate possible use cases of the extracted side-channel information. %damage from using the information provided by the \ATTCKNF algorithms.
\hltodo{to be removed.}
}
\label{fig:paper_overview}
\vspace{-1\baselineskip}
\end{figure*}


Safety critical systems such as self-driving cars, medicine/vaccine delivery drones, space rovers (\eg NASA's Opportunity and Spirit), industrial robots, autonomous tractors and military surveillance unmanned aerial vehicles (UAV), play a vital role in shaping today's technological evolution from everyday living to space exploration.
Such systems are often designed as real-time systems (RTS) consisting of real-time tasks\footnote{A task in typical real-time systems corresponds to a process/thread in generic operating systems. In this paper, we will use ``task'' and ``process'' interchangeably.} delivering time-sensitive functionality (\eg system heartbeat keepers, PID control processes, sensor data collectors, motor actuators). 
As these systems typically serve as critical infrastructures, they are prone to attacks (\eg Stuxnet~\cite{stuxnet:symantecdossier11}, BlackEnergy~\cite{khan2016threat}, attacks on automotive systems~\cite{checkoway2011comprehensive, woo2015practical}).
Furthermore, since critical cyber-physical systems tend to be heavily customized, malicious actors may spend significant time and resources in the reconnaissance stage to gather important information about the operation of the system before launching an actual, major attack~\cite{tankard2011advanced,
virvilis2013big}.
For instance, it has been reported that attackers had penetrated and stayed resident undetected in the system for {\em months} before they initiated the actual attack in the case of Stuxnet~\cite{stuxnet:symantecdossier11}. 
Once they had enough information about the precise nature of the system, they were able to craft effective attacks that were tailored to that particular system. 
%
As we point out in this paper, there exists a scheduler side-channel in the commonly deployed preemptive, fixed-priority RTS~\cite{Buttazzo:1997:HRC,LiuLayland1973,Liu:2000:RTS}, that can leak valuable timing behaviors of critical, high-priority, periodic real-time task(s) to unprivileged low-priority tasks. 
As a result, this scheduler side-channel and the leaked information are particularly useful in the reconnaissance stage of an attack to help mount a greater attack.
%real-time task scheduler~\cite{Buttazzo:1997:HRC,LiuLayland1973}

Real-time tasks are usually constrained by their predefined periods, deadlines, the worst-case execution times (WCET) and real-time scheduling algorithms (\eg fixed-priority preemptive scheduling, earliest deadline first scheduling~\cite{LiuLayland1973}).
These real-time constraints help system designers analyze the system as a whole and ensure that all safety guarantees are met (\eg no real-time tasks will miss their deadlines).
As a result, the system schedule (even a mix of both real-time and non-real-time tasks) becomes highly predicable.
This predictability, though favorable for the system analysis and safety, is a double-edged sword. % -- it creates side-channels in the real-time task scheduler.
A smart attacker can exploit the scheduler side-channels and the predictable nature of the system schedule to recover execution behaviors of the targeted tasks (that we call ``victim'' tasks) {\em at runtime} (our attack algorithms achieve exactly that). 
Knowing the precise schedule of the victim real-time tasks enables the attacker to pinpoint their future execution patterns.
%that can create attacker's interest to the fullest extent when launching a greater attack later.
%and launch greater attacks to gain even more information or cause the damage to the fullest extent.
The adversary can then launch more devastating attacks at those future execution points of victim tasks.
%In this paper, we present novel scheduler side-channel attack algorithms that take advantage of the predicable nature of the real-time tasks to gather and extract information about their precise timing behavior.


While most RTS with real-time tasks are vulnerable to the scheduler side-channel attacks presented in this paper, it is not trivial to learn and extract the exact times that the victim tasks are scheduled at {\em runtime}. 
In Section~{\ref{sec::discussion}}, we show that other existing analysis techniques cannot trivially handle this problem.
It is because \ci the actual schedule depends on the system start-up and initialization and other environmental conditions and \cii 
there may be multiple real-time and non-real-time tasks other than the victim task in the system that contribute to the uncertainty of the runtime schedule.  In other words, even knowledge of all the predefined parameters (\ie periods, deadlines and WCET) of all tasks alone is insufficient to reconstruct the actual schedule. 
While a privileged attacker might be able to extract the schedule directly from the scheduler, here we show that even an unprivileged attacker is able to learn the schedule of the victim task by using the proposed attack algorithms. 

In this paper, we present novel attack algorithms, named ``\ATTCK'', that exploit the scheduler side-channel in RTS.
We show that this side-channel can be exploited by %an unprivileged 
a malicious/compromised low-priority task (that we call a ``observer'' task), by simply observing its own execution intervals (\ie when the low-priority task itself is running and when it isn't).
It is important to note that scheduler covert channels where two processes covertly communicate using the scheduler have long been known (\eg~\cite{embeddedsecurity:volp2008, ghassami2015capacity, embeddedsecurity:son2006}). In contrast, our focus is on a side-channel that leaks execution timing behavior of critical, high-priority real-time tasks to any unprivileged, low-priority tasks.
%
With the \ATTCKNF algorithms, we are able to reconstruct the precise execution schedule of a periodic real-time victim task in the system by leveraging a compromised lower-priority user-space task. 
The \ATTCKNF algorithms can carry out the attack while \emph{staying within the execution time limits} of the compromised task.
%to reduce chances of detection and \hl{as such are particularly suitable for conducting reconnaissance and gathering information before launching more targeted attacks.}
It is particularly crucial for the attacker to not perturb the strict timing properties of the real-time autonomous control system, especially in the stage of reconstructing the information. %for the real-time tasks. 
Failing this will likely cause critical real-time functionality to fail or trigger a watchdog timeout that resets the system, leading to pre-mature detection of the attacker.


The \ATTCKNF algorithms are implemented on both a simulator and real hardware platforms 
running Real-time Linux and FreeRTOS (for the two attack 
case studies presented in Section~\ref{sec:casestudies}). We evaluate the
performance and scalability of \ATTCKNF in Section~\ref{sec::eval}, along with
a design space exploration (on the simulator). The results show that our methods are
effective at reconstructing schedule information and provide valuable
information for later attacks to better accomplish their attack goals.  To
summarize, the main contributions are: 
%\vspace{-0.5\baselineskip}
\begin{tight_enumerate}
\item Novel scheduler side-channel attack algorithms that can accurately
reconstruct the execution timing behaviors of critical real-time
tasks in real-time systems (without
requiring privileged access) [Section~\ref{sec::approach}]

\item Analyses and metrics to measure the accuracy in predicting the execution
and timing properties of the victim tasks [Section~\ref{sec::analysis}
and Section~\ref{sec::eval}].

\item \hl{Implementations and case studies on real hardware platforms} (\ie autonomous systems) running Real-time Linux and FreeRTOS [Section~{\ref{sec:casestudies}}].
\end{tight_enumerate}

 
